Digital identity architectures: comparing goals and vulnerabilities

Digital identity systems have the promise of efficiently facilitating access to services for a nation's citizens while increasing security and convenience. There are many possible system architectures, each with strengths and weaknesses that should be carefully considered. This report first establishes a set of goals and vulnerabilities faced by any identity system, then evaluates the trade-offs of common digital identity architectures, principally comparing centralised and decentralised systems.

==> branding/contents.tex <==
\newpage

\vspace*{1cm}
\tableofcontents

\newpage

==> branding/docrecord.tex <==
\newpage

\vspace*{1cm}
  
\large
\section*{Document preparation and Issue Record}

\vspace{1.5cm}
\begin{table}[htb]
\begin{tabular}{p{1cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
Version & Prepared & Reviewed & Approved & Issue Data & Issue Status \\
\midrule
2 & Callum Mole & Mark Hooper &     &   &  \\ \greyrule
    &   &   &   &   & \\ \greyrule
    &   &   &   &   & \\ \greyrule
    &   &   &   &   & \\ 
\bottomrule
\end{tabular}
\end{table}


==> branding/titlepage.tex <==
\begin{titlepage}
    
    %values arrived through trial and error
    {\transparent{.5}\includegraphics[width=1.15\textwidth,set height=2.9cm,left=\textwidth]{branding/banner.png}}
    
    \vspace*{1cm}
    
    \LARGE    
    \noindent Trusted Digital Infrastructure for Identity Systems    
    
    \vspace{2cm}

    \titlecolor
    \Huge
    {\fontfamily{\titlefont}\selectfont %separate font for title.
    \noindent\textbf{Summary Report:}
    
    %\vspace{.5cm}
    \noindent \textbf{Comparing platform architectures in \\ Digital Identity: goals met and \\ vulnerabilities faced}
        
    \vspace{1cm}
    \Large
    \noindent Research Engineering Group

    \noindent Jon Crowcroft, Principal Investigator
    
    \normalsize 
    \noindent December 2020
    }
    
    \normalsize
    \color{black}
    \vspace{3.5cm}
    \noindent Enquires:
    
    \noindent Mark Hooper \\
    mhooper@turing.ac.uk
    
    \noindent The Alan Turing Institute \\
    British Library \\
    96 Euston Road \\
    London \\
    NW1 2DB
    
\end{titlepage}

==> frontmatter.tex <==
\input{branding/titlepage}
\input{branding/docrecord}
\input{branding/contents}
